Ellipsoidal billiards in pseudo-Euclidean spaces and relativistic quadrics

We study geometry of confocal quadrics in pseudo-Euclidean spaces of an arbitrary dimension $d$ and any signature, and related billiard dynamics. The goal is to give a complete description of periodic billiard trajectories within ellipsoids. The novelty of our approach is based on introduction of a new discrete combinatorial-geometric structure associated to a confocal pencil of quadrics, a colouring in $d$ colours, by which we decompose quadrics of $d+1$ geometric types of a pencil into new relativistic quadrics of $d$ relativistic types. Deep insight of related geometry and combinatorics comes from our study of what we call discriminat sets of tropical lines $\Sigma^+$ and $\Sigma^-$ and their singularities. All of that enable usto get an analytic criterion describing all periodic billiard trajectories, including the light-like ones as those of a special interest.

==> 3-plane/confocal.tex <==
Here, we give a review of basic properties of families of confocal
conics in the Minkowski plane.

Denote by
\begin{equation}\label{eq:ellipse}
\mathcal{E}\ :\ \frac{x^2}{a}+\frac{y^2}{b}=1
\end{equation}
an ellipse in the plane, with $a$, $b$ being fixed positive numbers.

The associated family of confocal conics is:
\begin{equation}\label{eq:confocal.conics} 
\mathcal C_{\lambda}\ :\
\frac{x^2}{a-\lambda}+\frac{y^2}{b+\lambda}=1, \quad
\lambda\in\mathbf{R}.
\end{equation}

The family is shown on Figure \ref{fig:confocal.conics}.
\begin{figure}[h]
\input{0-figures/confocal_conics}
\caption{Family of confocal conics in the Minkowski
plane}\label{fig:confocal.conics}
\end{figure}
We may distinguish the following three subfamilies in the family
(\ref{eq:confocal.conics}):
\begin{itemize}
\item
for $\lambda\in(-b,a)$, conic $\mathcal{C}_{\lambda}$ is an ellipse;

\item
for $\lambda<-b$, conic $\mathcal{C}_{\lambda}$ is a hyperbola with $x$-axis as the major one;

\item
for $\lambda>a$, it is a hyperbola again, but now its major axis is $y$-axis.
\end{itemize}
In addition, there are three degenerated quadrics: 
\begin{itemize}
\item
$\mathcal{C}_{a}$ consists of the pair of points $F_1(\sqrt{a+b},0)$, $F_2(-\sqrt{a+b},0)$; 

\item
$\mathcal{C}_{b}$ is pair $G_1(0,\sqrt{a+b})$, $G_2(0,-\sqrt{a+b})$; and 

\item
$\mathcal{C}_{\infty}$ is pair $H_1(1:-1:0)$, $H_2(1:1:0)$ on the line at the infinity.
\end{itemize}
We notice four distinguished lines: 
$$
x+y=\sqrt{a+b},\ x+y=-\sqrt{a+b},\ x-y=\sqrt{a+b},\ x-y=-\sqrt{a+b}.
$$
These lines
are common tangents to all the conics from the confocal family.

It is elementary and straightforward to prove the following
\begin{proposition}
For each point on ellipse $\mathcal{C}_{\lambda}$, $\lambda\in(-b,a)$,
either sum or difference of its Minkowski distances from the foci $F_1$ and
$F_2$ is equal to $2\sqrt{a-\lambda}$;
either sum or difference
of the distances from the other pair of foci $G_1$, $G_2$ is equal to $2i\sqrt{b+\lambda}$.

Either sum or difference of the Minkowski distances of each point of hyperbola
$\mathcal{C}_{\lambda}$, $\lambda\in(-\infty,-b)$, from the foci
$F_1$ and $F_2$ is equal to $2\sqrt{a-\lambda}$;
for the other pair of foci $G_1$, $G_2$, it is
equal to $2\sqrt{-b-\lambda}$.

Either sum or difference of the Minkowski distances of each point of hyperbola
$\mathcal{C}_{\lambda}$, $\lambda\in(a,+\infty)$, from the foci
$F_1$ and $F_2$ is equal to $2i\sqrt{\lambda-a}$;
for the other pair of foci $G_1$, $G_2$, it is equal to $2i\sqrt{b+\lambda}$.
\end{proposition}

Billiard within an ellipse also have the famous focal property:

\begin{proposition}
Consider a billiard trajectory within ellipse $\mathcal{E}$ given by
equation (\ref{eq:ellipse}) in the Minkowski plane, such that the
line containing the initial segment of the trajectory passes through
a focus of the confocal family (\ref{eq:confocal.conics}), say
$F_1$, $G_1$, or $H_1$.
If the tangent line to $\mathcal{E}$ at the
reflection point of this segment is not light-like, then the line
containing the next segment will pass through $F_2$, $G_2$, or $H_2$
respectively.
\end{proposition}

In other words, the segments of one billiard trajectory will
alternately contain foci of one of the pairs $(F_1,F_2)$,
$(G_1,G_2)$, $(H_1,H_2)$. The only exception are successive segments
obtained by the reflection on the light-like tangent. Such segments
coincide.

